Exploiting Observation Bias to Improve Matrix Completion

We consider a variant of matrix completion where entries are revealed in a biased manner. We wish to understand the extent to which such bias can be exploited in improving predictions. Towards that, we propose a natural model where the observation pattern and outcome of interest are driven by the same set of underlying latent (or unobserved) factors. We devise Mask Nearest Neighbor (MNN), a novel two-stage matrix completion algorithm: first, it recovers (distances between) the latent factors by utilizing matrix estimation for the fully observed noisy binary matrix, corresponding to the observation pattern; second, it utilizes the recovered latent factors as features and sparsely observed noisy outcomes as labels to perform non-parametric supervised learning. Our analysis reveals that MNN enjoys entry-wise finite-sample error rates that are competitive with corresponding supervised learning parametric rates. Despite not having access to the latent factors and dealing with biased observations, MNN exhibits such competitive performance via only exploiting the shared information between the bias and outcomes. Finally, through empirical evaluation using a real-world dataset, we find that with MNN, the estimates have 28x smaller mean squared error compared to traditional matrix completion methods, suggesting the utility of the model and method proposed in this work.

==> 0.abstract.tex <==
\begin{abstract}

We consider a variant of matrix completion where entries are revealed in a biased manner, adopting a model akin to that introduced by Ma $\&$ Chen \citep{ma2019missing}. Instead of treating this observation bias as a disadvantage, as is typically the case, the goal is to exploit the shared information between the bias and the outcome of interest to improve predictions. Towards this, we consider a natural model where the observation pattern and outcome of interest are driven by the same set of underlying latent or unobserved factors. This leads to, Mask
Nearest Neighbor ($\MNN$), a two stage matrix completion algorithm: first, recover (distances between) the latent factors by utilizing matrix completion for the {\em fully} observed noisy binary matrix corresponding to the observation pattern; second, utilize the recovered latent factors as features and sparsely observed noisy outcomes as labels to perform non-parametric supervised learning. The finite-sample error rates analysis suggests that, ignoring logarithmic factors, this approach is competitive with the corresponding supervised learning parametric rates. This implies the $\MNN$ method has performance that is comparable to having access to the \emph{unobserved} latent factors through exploiting the shared information between the bias and outcomes. Unlike related recent work \cite{agarwal2021causal}, the proposed method is computationally efficient. Through empirical evaluation using a real-world dataset, we find that with this $\MNN$, the estimates have 28x smaller mean squared error compared to traditional matrix completion methods, suggesting the utility of the model and the method proposed in this work. 

    % We consider a variant of matrix completion where entries are revealed in a biased manner, adopting a model akin to that introduced by \citet{ma2019missing}. Instead of treating this observation bias as a disadvantage, as is typically the case, the goal is to exploit the shared information between the bias and the outcome of interest to improve predictions. Towards this, we consider a natural model where the observation pattern and outcome of interest are driven by the same set of underlying latent or unobserved factors. This leads to a two stage matrix completion algorithm: first, recover (distances between) the latent factors by utilizing matrix completion for the {\em fully} observed noisy binary matrix corresponding to the observation pattern; second, utilize the recovered latent factors as features and sparsely observed noisy outcomes as labels to perform non-parametric supervised learning to de-noise the observed outcomes and predict the unobserved outcomes. The finite-sample error rates analysis suggest that, ignoring logarithmic factors, this approach is competitive with the corresponding supervised learning parametric rates. That is, the two-stage method has performance that is comparable to having access to the \emph{unobserved} or {\em latent} factors. And it is because of the ability to exploit the relationship between observation pattern and outcomes through the shared latent factors carefully. Indeed, through empirical evaluation using a real-world dataset we find that with this two-stage algorithm, the estimates have 30x smaller mean squared error compared to traditional matrix completion methods suggesting the utility of the model and the method proposed in this work. 

    % We consider a variant of matrix completion where entries are revealed in a biased manner, adopting a model akin to that introduced by \citet{ma2019missing}. Instead of treating this observation bias as a disadvantage, as is typically the case, our goal is to exploit the shared information between the bias and the outcome of interest to improve predictions. Towards this, we propose a simple two-stage algorithm: (i) interpreting the observation pattern as a fully observed noisy matrix, we apply traditional matrix completion methods to the observation pattern to estimate the distances between the latent factors; (ii) we apply supervised learning on the recovered latent factors (as features) to impute missing observations. We establish finite-sample error rates that are, ignoring logarithmic factors, competitive with the corresponding supervised learning parametric rates, suggesting that our learning performance is comparable to having access to the \emph{unobserved} or {\em latent} factors. Empirical evaluation using a real-world dataset reflects similar performance gains, with our algorithm's estimates having 30x smaller mean squared error compared to traditional matrix completion methods. 

    
\end{abstract}
